A novel switched systems approach to nonconvex optimisation

We develop a novel switching dynamics that converges to the Karush-Kuhn-Tucker (KKT) point of a nonlinear optimisation problem. This new approach is particularly notable for its lower dimensionality compared to conventional primal-dual dynamics, as it focuses exclusively on estimating the primal variable. Our method is successfully illustrated on general quadratic optimisation problems, the minimisation of the classical Rosenbrock function, and a nonconvex optimisation problem stemming from the control of energy-efficient buildings.

==> images/correctionFunction.tex <==
\begin{figure}[htb]
    \begin{tikzpicture}
        \begin{axis}[
            axis x line=center,
            axis y line=center,
            xlabel style={below right},
            ylabel style={above},
            xmin=0,
            xmax=2.38,
            ymin=-0.25,
            ymax=1.35,
            minor xtick={1,2,3},
            minor ytick={1},
            grid=minor,
            xlabel=time $t$,
            ylabel={$h_\sigma(\sigma(t),t)$},
            %xtick={1,2,3},
            xtick={0.2,0.3,0.9,1,1.2,1.3,1.9,2,2.3,2.4,2.5,3},
            xticklabels={$t_1$,$t_2$,$t_3$,$t_4$,$t_5$,$t_6$,$t_7$,$t_8$,$t_9$,$t_{10}$,$t_{11}$,$t_{12}$},
            xticklabel style={font=\tiny},
            %minor x tick label style = {font=\tiny},
            extra x ticks ={0.5,1.5,2.5},
            extra x tick labels={${\sigma(t) \in \mathcal S}$, $\sigma(t) \in \mathcal U$, $\sigma(t) \in \mathcal S$},
            extra x tick style={% ändern des Stils für extraticks
                every tick/.append style={draw=none},% andere Farbe und Breite
                %major tick length=1cm% andere Länge
                xticklabel style = {font=\normalsize,yshift=-.3cm}
            },
            ytick={0,1},
			yticklabels=\empty,
            ymajorgrids=true,
            extra y ticks={0,1},
            extra y tick labels={{\tiny${-T_{\mathcal S}(1 - \delta)\quad}$ ${-T_{\mathcal U}(1 + \delta)}$},0},
            yticklabel style={text width=1.4cm,align=right},
            width=.85\columnwidth,
            height=.75\columnwidth,
            set layers=tick labels on top
            ]
            % fade out background behind axis labels
            \draw[draw=none,fill=white] (0.1,-0.05) rectangle (3.2,-0.14);

            % stable flow
            \draw[color=customblue,thick,smooth] (0,1)--(0.2,1)(0.2,0.8)--(0.3,0.9)(0.3,0.7)--(0.6,1)--(0.9,1)(0.9,0.8)--(1,0.9);
            \addplot[mark=*,only marks,color=customblue,forget plot] coordinates {(0.2,0.8)(0.3,0.7)(0.9,0.8)};
            \addplot[mark=*,fill=white,only marks,draw=customblue,thick,forget plot] coordinates {(0.2,1)(0.3,0.9)(0.9,1)(1,0.9)};
            \draw[dotted,color=customblue,thick,smooth] (0.2,1)--(0.2,0.8)(0.3,0.9)--(0.3,0.7)(0.9,1)--(0.9,0.8);
            % stable jump
            \draw[color=customblue,thick,smooth] (1,0.7)--(1.2,0.5)(1.2,0.9)--(1.3,0.8)(1.3,1)--(1.9,0.4)(1.9,0.8)--(2,0.7);
            \addplot[mark=*,only marks,color=customblue,forget plot] coordinates {(1,0.7)(1.2,0.9)(1.3,1)(1.9,0.8)};
            \addplot[mark=*,fill=white,only marks,draw=customblue,thick,forget plot] coordinates {(1.2,0.5)(1.3,0.8)(1.9,0.4)(2,0.7)};
            \draw[dotted,color=customblue,thick,smooth] (1,0.9)--(1,0.7)(1.2,0.5)--(1.2,0.9)(1.3,0.8)--(1.3,1)(1.9,0.4)--(1.9,0.8);
            % stable flow
            \draw[color=customblue,thick,smooth] (2,1)--(2.3,1)(2.3,0.8)--(2.4,0.9)(2.4,0.7)--(2.5,0.8)(2.5,0.6)--(2.9,1)--(3,1);
            \addplot[mark=*,only marks,color=customblue,forget plot] coordinates {(2,1)(2.3,0.8)(2.4,0.7)(2.5,0.6)};
            \addplot[mark=*,fill=white,only marks,draw=customblue,thick,forget plot] coordinates {(2.3,1)(2.4,0.9)(2.5,0.8)};
            \draw[dotted,color=customblue,thick,smooth] (2,0.7)--(2,1)(2.3,1)--(2.3,0.8)(2.4,0.9)--(2.4,0.7)(2.5,0.8)--(2.5,0.6);
            % unstable flow
            \draw[color=customblue,thick,smooth] (3,0.8)--(3.3,0.5);
            \addplot[mark=*,only marks,color=customblue,forget plot] coordinates {(3,0.8)};
            \addplot[mark=*,fill=white,only marks,draw=customblue,thick,forget plot] coordinates {(3,1)};
            \draw[dotted,color=customblue,thick,smooth] (3,1)--(3,0.8);

            \draw [decorate, decoration = {brace,raise=3pt}] (0.9,0.8)--(0.9,1);
            \node at (0.68,0.85) {\footnotesize$\tau_{\sigma(t_3^-)}$};
            
            \draw [decorate, decoration = {brace,raise=3pt}] (1.9,0.8)--(1.9,0.4);
            \node at (2.17,0.57) {\footnotesize$\tau_{\sigma(t_7^-)}$};
     
            %\legend{${V(t,x(t))}$, ${W(t,x(t))}$};
        \end{axis}
    \end{tikzpicture}        
	\caption{Illustration of function $h_\sigma(p,t)$ for a fixed switching signal.\label{fig:correctionFunction}}
\end{figure}


==> images/decrLF.tex <==
\begin{figure}[htb]
    \begin{tikzpicture}
        \begin{axis}[
            axis x line=center,
            axis y line=center,
            xlabel style={below right},
            ylabel style={above},
            minor xtick={1,2,3},
            grid=minor,
            xmin=0,
            xmax=3.1,
            ymin=-0.35,
            ymax=1.35,
            xlabel=time $t$,
            ylabel={$V_\sigma$, $W_\sigma$},
            xtick={1,2,3},
            xticklabels={$t_1$,$t_2$,$t_3$},
            xticklabel style={font=\tiny},
            %xticklabel style = {font=\footnotesize},
            extra x ticks ={0.5,1.5,2.5},
            %xtick style={draw=white},
            extra x tick labels={${\sigma(t) \in \mathcal S}$, $\sigma(t) \in \mathcal U$, $\sigma(t) \in \mathcal S$},
            extra x tick style={% ändern des Stils für extraticks
                every tick/.append style={draw=none},% andere Farbe und Breite
                %major tick length=1cm% andere Länge
                xticklabel style = {font=\normalsize,yshift=-.3cm}
            },
            ytick=\empty,
            width=.95\columnwidth,
            height=.60\columnwidth,
            set layers=tick labels on top
            ]
            % fade out background behind axis labels
            \draw[draw=none,fill=white] (0.1,-0.07) rectangle (3.2,-0.18);
            
            % non-decreasing Lyapunov function
            \addplot[domain=0:1,color=customblue,thick,smooth] {exp(-1.2*x)};
            \addplot[domain=1:2,color=customblue,thick,smooth,forget plot] {exp(+0.2*x-0.7)};
            \addplot[domain=2:3,color=customblue,thick,smooth,forget plot] {exp(-2*x+3)};
            \addplot[domain=3:3.25,color=customblue,thick,smooth,forget plot] {exp(+0.2*x-2.1)};
            \addplot[mark=*,only marks,color=customblue,forget plot] coordinates {(1,{exp(-0.5)})(2,{exp(-1)})(3,{exp(-1.5)})};
            \addplot[mark=*,fill=white,only marks,draw=customblue,thick,forget plot] coordinates {(1,{exp(-1.2)})(2,{exp(-0.3)})(3,{exp(-3)})};
            \draw[dotted,color=customblue,thick,smooth] (1,{exp(-0.5)})--(1,{exp(-1.2)});
            \draw[dotted,color=customblue,thick,smooth] (2,{exp(-1)})--(2,{exp(-0.3)});
            \draw[dotted,color=customblue,thick,smooth] (3,{exp(-1.5)})--(3,{exp(-3)});
            
            % decreasing Lyapunov function
            \addplot[color=red,thick,smooth] {exp(-0.5*x)};
            
            \legend{${V_\sigma(t,x(t))}$, ${W_\sigma(t,x(t))}$};
        \end{axis}
    \end{tikzpicture}
	\caption{Construction of a decreasing ISS-Lyapunov function $W_\sigma(t,x(t))$ from a non-decreasing ISS-Lyapunov function $V_\sigma(t,x(t))$ and their relation.\label{fig:decrLF}}
\end{figure}

